IceCube search for neutrinos from novae

Despite being one of the longest known classes of astrophysical transients, novae continue to present modern surprises. The Fermi-LAT discovered that many if not all novae are GeV gamma ray sources, even though theoretical models had not even considered them as a possible source class. More recently, MAGIC and H.E.S.S. detected TeV gamma rays from a nova. Moreover, there is strong evidence that the gamma rays are produced hadronically, and that the long-studied optical emission by novae is also shock-powered. If this is true, novae should emit a neutrino signal correlated with their gamma-ray and optical signals. We present the first search for neutrinos from novae. Because the neutrino energy spectrum is expected to match the gamma-ray spectrum, we use an IceCube DeepCore event selection focused on GeV-TeV neutrinos. We present results from two searches, one for neutrinos correlated with gamma-ray emission and one for neutrinos correlated with optical emission. The event selection presented here is promising for additional astrophysical transients including gamma-ray bursts and gravitational wave sources.

==> gamma_ray_results_w_rsoph.tex <==
\begin{table*}
\centering
    %make table fit in margins
    \tabcolsep=5.5pt\relax
    \small
\begin{tabular}{ccccccccccc}
\toprule
Name &                 $\alpha$ & $\delta$ & MJD$_{\mathrm{start}}$ & MJD$_{\mathrm{stop}}$ &  $\Delta$T & TS & $\hat{n}_{s}$ &$\hat{\gamma}$ &   pre-trial & $E^2F$ @ 1~TeV \\
&  &  & &  &(days)  &  & & &   $p$-value & (GeV cm$^{-2}$)\\
\midrule
V1324 Sco & 267.7$^{\circ}$ & -32.6$^{\circ}$ &                56093.0 &               56110.0 & 17.0 &         0.00 &                     0.0& -- & 1.000 & 26.4\\
 V959 Mon &   99.9$^{\circ}$ & +5.9$^{\circ}$ &                56097.0 &               56119.0 & 22.0 &         1.14 &                  14.8& 2.75 & 0.197 & 9.76\\
 V339 Del & 305.9$^{\circ}$& +20.8$^{\circ}$ &                56520.0 &               56547.0 & 27.0 &         0.00 &                     0.0& -- & 1.000 & 2.10\\
V1369 Cen & 208.7$^{\circ}$& -59.2$^{\circ}$ &                56634.0 &               56672.0 & 38.0 &          0.01 &                   3.8& 4.00 & 0.070 & 62.9\\
 V745 Sco & 268.8$^{\circ}$& -33.2$^{\circ}$ &                56694.0 &               56695.0 & 1.0 &         0.00 &                     0.0& -- & 1.000 & 7.45\\
V1535 Sco & 255.9$^{\circ}$& -35.1$^{\circ}$ &                57064.0 &               57071.0 & 7.0 &         6.95 &                  59.9& 3.02 & 0.002 & 42.6\\
V5668 Sgr & 279.2$^{\circ}$& -28.9$^{\circ}$ &                57105.0 &               57158.0 &  53.0 &        1.30 &                  62.0& 3.16 & 0.112 & 69.6\\
 V407 Lup & 232.3$^{\circ}$& -44.8$^{\circ}$ &                57657.0 &               57660.0 & 3.0 &         0.00 &                     0.0& -- & 1.000 & 11.2\\
V5855 Sgr & 272.6$^{\circ}$& -27.5$^{\circ}$ &                57686.0 &               57712.0 & 26.0 &           0.00 &                     0.0& -- & 1.000 & 28.3\\
V5856 Sgr & 275.2$^{\circ}$& -28.4$^{\circ}$ &                57700.0 &               57715.0 & 15.0 &          5.13 &                  40.3& 2.81 & 0.015 & 47.0\\
 V549 Vel & 132.6$^{\circ}$& -47.8$^{\circ}$ &                58037.0 &               58070.0 & 33.0 &          0.22 &                  22.4& 4.00 & 0.062 & 51.6\\
 V357 Mus & 171.6$^{\circ}$& -65.5$^{\circ}$ &                58129.0 &               58156.0 & 27.0 &          0.01 &                   5.0& 4.00 & 0.115 & 52.3\\
 V906 Car & 159.1$^{\circ}$& -59.6$^{\circ}$ &                58216.0 &               58239.0 & 23.0 &         0.00 &                     0.0& -- & 1.000 & 36.5\\
 V392 Per &  70.8$^{\circ}$& +47.4$^{\circ}$ &                58238.0 &               58246.0 & 8.0 &          0.88 &                  15.4& 3.64 & 0.373 & 1.92\\
V3890 Sgr & 277.7$^{\circ}$& -24.0$^{\circ}$ &                58718.0 &               58739.0 & 21.0 &          0.00 &                     0.0& -- & 1.000 & 22.6\\
V1707 Sco & 264.3$^{\circ}$& -35.2$^{\circ}$ &                58740.0 &               58744.0 & 4.0 &          0.00 &                     0.0& -- & 1.000 & 10.6\\
RS Oph & 267.6$^{\circ}$ & -6.7$^{\circ}$ & 59434.8 & 59464.8 & 30.0 & 0.28 & 3.8 & 2.4 & 0.255 & 16.1 \\\
\bottomrule
\end{tabular}
\caption{Results from the gamma-ray correlation analysis. MJD$_{\mathrm{start}}$ and MJD$_{\mathrm{stop}}$ represent the beginning and end of when a nova was detected by \textit{Fermi}-LAT, respectively. This is the same time window used for the neutrino search. The observed test statistic (TS), best-fit number of signal events ($\hat{n}_{s}$) and best-fit spectral index ($\hat{\gamma}$) for the neutrino search from each nova are given here. The $p$-values shown are before accounting for the factor accrued from performing multiple searches. The final column gives the time-integrated flux upper limit for each nova, assuming a power-law spectrum with a spectral index of 2.0 ($dN/dE \propto E^{-2}$) and including the systematic uncertainty as discussed in \cite[Section 4.3]{IceCube:2022lnv}.}
\label{tab:gamma_results}
\end{table*}

